Say What I Want: Towards the Dark Side of Neural Dialogue Models

Neural dialogue models have been widely adopted in various chatbot applications because of their good performance in simulating and generalizing human conversations. However, there exists a dark side of these models -- due to the vulnerability of neural networks, a neural dialogue model can be manipulated by users to say what they want, which brings in concerns about the security of practical chatbot services. In this work, we investigate whether we can craft inputs that lead a well-trained black-box neural dialogue model to generate targeted outputs. We formulate this as a reinforcement learning (RL) problem and train a Reverse Dialogue Generator which efficiently finds such inputs for targeted outputs. Experiments conducted on a representative neural dialogue model show that our proposed model is able to discover such desired inputs in a considerable portion of cases. Overall, our work reveals this weakness of neural dialogue models and may prompt further researches of developing corresponding solutions to avoid it.

==> abs.tex <==
Neural dialogue models have been widely adopted in various chatbot applications because of their good performance in simulating and generalizing human conversations. However, there exists a dark side of these models -- due to the vulnerability of neural networks, a neural dialogue model can be manipulated by users to say what they want, which brings in concerns about the security of practical chatbot services. In this work, we investigate whether we can craft inputs that lead a well-trained black-box neural dialogue model to generate targeted outputs. We formulate this as a reinforcement learning (RL) problem and train a Reverse Dialogue Generator which efficiently finds such inputs for targeted outputs. Experiments conducted on a representative neural dialogue model show that our proposed model is able to discover such desired inputs in a considerable portion of cases. Overall, our work reveals this weakness of neural dialogue models and may prompt further researches of developing corresponding solutions to avoid it.

==> references.tex <==
% \section*{References}

% % References follow the acknowledgments. Use unnumbered first-level heading for
% % the references. Any choice of citation style is acceptable as long as you are
% % consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
% % when listing the references. {\bf Remember that you can use more than eight
% %   pages as long as the additional pages contain \emph{only} cited references.}
% % \medskip

% \small

% [1] Ritter, A., Cherry, C.,\ \& Dolan, W. B.\ (2011, July). Data-driven response generation in social media. In {\it Proceedings of the conference on empirical methods in natural language processing} (pp. 583-593). Association for Computational Linguistics.



% [2] Weizenbaum, J.\ (1966). ELIZA---a computer program for the study of natural language communication between man and machine. {\it Communications of the ACM}, 9(1), 36-45.

% [3] Goddeau, D., Meng, H., Polifroni, J., Seneff, S.,\ \& Busayapongchai, S. (1996, October). A form-based dialogue manager for spoken language applications. In {\it Proceeding of Fourth International Conference on Spoken Language Processing. ICSLP'96} (Vol. 2, pp. 701-704). IEEE.

% [4] Lester, J., Branting, K.,\ \& Mott, B.\ (2004). Conversational agents. {\it The Practical Handbook of Internet Computing}, 220-240.

% [5] Jurafsky, D.,\ \& Martin, J. H.\ (2014). {\it Speech and language processing} (Vol. 3). London: Pearson.

% [6] Banchs, R. E.\ (2012). Movie-DiC: a movie dialogue corpus for research and development. In {\it Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers} (Vol. 2, pp. 203-207).

% [7] Ameixa, D., Coheur, L., Fialho, P.,\ \& Quaresma, P.\ (2014, August). Luke, I am your father: dealing with out-of-domain requests by using movies subtitles. {\it In International Conference on Intelligent Virtual Agents} (pp. 13-21). Springer, Cham.

% [8] Lu, Z.,\ \& Li, H.\ (2013). A deep architecture for matching short texts. In {\it Advances in neural information processing systems} (pp. 1367-1375).

% [9] Hu, B., Lu, Z., Li, H.,\ \& Chen, Q.\ (2014). Convolutional neural network architectures for matching natural language sentences. In {\it Advances in neural information processing systems} (pp. 2042-2050).

% [10] Song, Y., Yan, R., Li, X., Zhao, D.,\ \& Zhang, M.\ (2016). Two are better than one: An ensemble of retrieval-and generation-based dialog systems. {\it arXiv preprint arXiv:1610.07149}.

% [11] Gao, J., Galley, M.,\ \& Li, L.\ (2019). Neural approaches to conversational AI. {\it Foundations and Trends® in Information Retrieval}, 13(2-3), 127-298.

% [12] Sutskever, I., Vinyals, O.,\ \& Le, Q. V.\ (2014). Sequence to sequence learning with neural networks. In {\it Advances in neural information processing systems} (pp.\ 3104-3112).

% [13] Sordoni, A., Galley, M., Auli, M., Brockett, C., Ji, Y., Mitchell, M., ...\ \& Dolan, B.\ (2015). A neural network approach to context-sensitive generation of conversational responses. {\it arXiv preprint arXiv:1506.06714}.

% [14] Vinyals, O.,\ \& Le, Q.\ (2015). A neural conversational model. {\it arXiv preprint arXiv:1506.05869}.

% [15] Shang, L., Lu, Z.,\ \& Li, H. (2015). Neural responding machine for short-text conversation. {\it arXiv preprint arXiv:1503.02364}.

% [16] Serban, I. V., Sordoni, A., Bengio, Y., Courville, A.,\ \& Pineau, J.\ (2016, March). Building end-to-end dialogue systems using generative hierarchical neural network models. In {\it Thirtieth AAAI Conference on Artificial Intelligence}.

% [17] Serban, I. V., Sordoni, A., Lowe, R., Charlin, L., Pineau, J., Courville, A.,\ \& Bengio, Y.\ (2017, February). A hierarchical latent variable encoder-decoder model for generating dialogues. In {\it Thirty-First AAAI Conference on Artificial Intelligence}.

% [18] Zhou, L., Gao, J., Li, D.,\ \& Shum, H. Y.\ (2018). The Design and Implementation of XiaoIce, an Empathetic Social Chatbot. {\it arXiv preprint arXiv:1812.08989}.

% [19] Szegedy, C., Zaremba, W., Sutskever, I., Bruna, J., Erhan, D., Goodfellow, I.,\ \& Fergus, R.\ (2013). Intriguing properties of neural networks. {\it arXiv preprint arXiv:1312.6199}.

% [20] Yuan, X., He, P., Zhu, Q.,\ \& Li, X.\ (2019). Adversarial examples: Attacks and defenses for deep learning. {\it IEEE transactions on neural networks and learning systems}.

% [21] Wolf, M. J., Miller, K.,\ \& Grodzinsky, F. S.\ (2017). Why we should have seen that coming: comments on Microsoft's tay experiment, and wider implications. {\it ACM SIGCAS Computers and Society}, 47(3), 54-64.

% [22] Price, R.\ (2016). Microsoft is deleting its AI chatbot’s incredibly racist tweets. {\it Business Insider}.

% [23] He, T.,\ \& Glass, J.\ (2018). Detecting egregious responses in neural sequence-to-sequence models. arXiv preprint {\it arXiv:1809.04113}.

% [24] Chen, H., Zhang, H., Chen, P. Y., Yi, J.,\ \& Hsieh, C. J.\ (2017). Attacking visual language grounding with adversarial examples: A case study on neural image captioning. {\it arXiv preprint arXiv:1712.02051}.

% [25] Sharif, M., Bhagavatula, S., Bauer, L.,\ \& Reiter, M. K.\ (2016, October). Accessorize to a crime: Real and stealthy attacks on state-of-the-art face recognition. In {\it Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security} (pp. 1528-1540). ACM.

% [26] Xie, C., Wang, J., Zhang, Z., Zhou, Y., Xie, L.,\ \& Yuille, A.\ (2017). Adversarial examples for semantic segmentation and object detection. In {\it Proceedings of the IEEE International Conference on Computer Vision} (pp. 1369-1378).

% [27] Kos, J., Fischer, I.,\ \& Song, D.\ (2018, May). Adversarial examples for generative models. In {\it 2018 IEEE Security and Privacy Workshops (SPW)} (pp. 36-42). IEEE.

% [28] Tabacof, P., Tavares, J.,\ \& Valle, E.\ (2016). Adversarial images for variational autoencoders. {\it arXiv preprint arXiv:1612.00155}.

% [29] Huang, S., Papernot, N., Goodfellow, I., Duan, Y.,\ \& Abbeel, P.\ (2017). Adversarial attacks on neural network policies. {\it arXiv preprint arXiv:1702.02284}.

% [30] Kos, J.,\ \& Song, D.\ (2017). Delving into adversarial attacks on deep policies. {\it arXiv preprint arXiv:1705.06452}.

% [31] Zhang, W. E., Sheng, Q. Z.,\ \& Alhazmi, A. A. F.\ (2019). Generating Textual Adversarial Examples for Deep Learning Models: A Survey. {\it arXiv preprint arXiv:1901.06796}.

% [32] Lei, Q., Wu, L., Chen, P. Y., Dimakis, A. G., Dhillon, I. S.,\ \& Witbrock, M.\ (2018). Discrete attacks and submodular optimization with applications to text classification. {\it arXiv preprint arXiv:1812.00151}.

% [33] Liang, B., Li, H., Su, M., Bian, P., Li, X., & Shi, W. (2017). Deep text classification can be fooled. {\it arXiv preprint arXiv:1704.08006}.

% [34] Iyyer, M., Wieting, J., Gimpel, K.,\ \& Zettlemoyer, L.\ (2018). Adversarial example generation with syntactically controlled paraphrase networks. {\it arXiv preprint arXiv:1804.06059}.

% [35] Sato, M., Suzuki, J., Shindo, H.,\ \& Matsumoto, Y.\ (2018). Interpretable adversarial perturbation in input embedding space for text. {\it arXiv preprint arXiv:1805.02917}.

% [36] Belinkov, Y.,\ \& Bisk, Y.\ (2017). Synthetic and natural noise both break neural machine translation. {\it arXiv preprint arXiv:1711.02173}.

% [37] Chan, A., Ma, L., Juefei-Xu, F., Xie, X., Liu, Y.,\ \& Ong, Y. S.\ (2018). Metamorphic Relation Based Adversarial Attacks on Differentiable Neural Computer. {\it arXiv preprint arXiv:1809.02444}.

% [38] Wieting, J., Bansal, M., Gimpel, K.,\ \& Livescu, K.\ (2015). Towards universal paraphrastic sentence embeddings. {\it arXiv preprint arXiv:1511.08198}.

% [39] Seq2Sick: Evaluating the Robustness of Sequence-to-Sequence Models with Adversarial Examples

% [40] A diversity-promoting objective function for neural conversation models
% % [1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
% % connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
% % (eds.), {\it Advances in Neural Information Processing Systems 7},
% % pp.\ 609--616. Cambridge, MA: MIT Press.

% % [2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
% %   Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
% % TELOS/Springer--Verlag.

% % [3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
% % recall at excitatory recurrent synapses and cholinergic modulation in rat
% % hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
